Graphon Signal Processing

Graphons are infinite-dimensional objects that represent the limit of convergent sequences of graphs as their number of nodes goes to infinity. This paper derives a theory of graphon signal processing centered on the notions of graphon Fourier transform and linear shift invariant graphon filters, the graphon counterparts of the graph Fourier transform and graph filters. It is shown that for convergent sequences of graphs and associated graph signals: (i) the graph Fourier transform converges to the graphon Fourier transform when the graphon signal is bandlimited; (ii) the spectral and vertex responses of graph filters converge to the spectral and vertex responses of graphon filters with the same coefficients. These theorems imply that for graphs that belong to certain families, i.e., that are part of sequences that converge to a certain graphon, graph Fourier analysis and graph filter design have well defined limits. In turn, these facts extend applicability of graph signal processing to graphs with large number of nodes -- since signal processing pipelines designed for limit graphons can be applied to finite graphs -- and to dynamic graphs -- since we can relate the result of SP pipelines designed for different graphs from the same convergent graph sequence.

==> figures/AggregationCNNGS/AggregationCNNGSParam.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{4}
\def\Yscale{0.125}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{PathNodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {32} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {10} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.6}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {8}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {8}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {2}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {2}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {1.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.2*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.7*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/AggregationCNNGS/AggregationCNNGSParamGraph.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{GraphNodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {100} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {80/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.2}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {30}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {5}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {1}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {5}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {3}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {2*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.2*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {3*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/AggregationCNNGS/GraphNodePositions.tex <==
\def \posXarray {{
0.47, 0.22, 0.78, 0.09, 0.81, 
0.63, 0.90, 0.99, 0.77, 0.70, 0.01, 0.61, 0.55, 0.04, 0.72, 0.98, 0.68, 0.57, 0.26, 0.23, 0.28, 0.06, 0.85, 0.89, 0.98, 
0.88, 0.26, 0.02, 0.14, 0.17, 0.20, 0.01, 0.68, 0.77, 0.05, 0.60, 0.60, 0.04, 0.50, 0.05, 0.49, 0.38, 0.85, 0.48, 0.49, 
0.28, 0.26, 0.80, 0.84, 0.71, 0.36, 0.22, 0.33, 0.10, 0.99, 0.04, 0.66, 0.20, 0.91, 0.21, 0.04, 0.26, 0.16, 0.25, 0.68, 
0.89, 0.92, 0.25, 0.45, 0.77, 0.31, 0.99, 0.09, 0.41, 0.45, 0.63, 0.19, 0.28, 0.58, 0.28, 0.72, 0.25, 0.80, 0.26, 0.61, 
0.19, 0.16, 0.09, 0.32, 0.08, 0.39, 0.04, 0.93, 0.83, 0.72, 0.81, 0.38, 0.94, 0.42, 0.66, 0.88, 0.30, 0.77, 0.58, 0.68, 
%0.64, 0.09, 0.35, 0.30, 0.75, 0.44, 0.40, 0.47, 0.77, 0.29, 0.41, 0.64, 0.27, 0.18, 0.77, 0.98, 0.97, 0.05, 0.45, 0.28, 
%0.65, 0.30, 0.17, 0.69, 0.60, 0.22, 0.68, 0.05, 0.61, 0.50, 0.50, 0.46, 0.76, 0.13, 0.73, 0.53, 0.31, 0.66, 0.49, 0.63, 
%0.35, 0.24, 0.81, 0.75, 0.37, 0.58, 0.57, 0.48, 0.73, 0.89, 0.16, 0.62, 0.44, 0.53, 0.82, 0.80, 0.02, 0.92, 0.16, 0.12, 
%0.19, 0.66, 0.75, 0.48, 0.17, 0.49, 0.50, 0.02, 0.40, 0.70, 0.39, 0.20, 0.32, 0.52, 0.31, 0.76, 0.29, 0.51, 0.66, 0.80, 
%0.16, 0.65, 0.13, 0.63, 0.35, 0.44, 0.06, 0.87, 0.23, 0.43, 0.13, 0.56, 0.36, 0.45, 0.25, 0.61, 0.26, 0.29, 0.99, 0.04
}}

\def \posYarray {{
0.52, 0.18, 0.22, 0.83, 0.78, 
0.03, 0.61, 0.08, 0.86, 0.33, 0.64, 0.99, 0.43, 0.50, 0.63, 0.63, 0.40, 0.51, 0.22, 0.06, 0.03, 0.19, 0.18, 0.23, 0.16, 
0.21, 0.19, 0.12, 0.35, 0.06, 0.28, 0.76, 0.66, 0.25, 0.62, 0.13, 0.72, 0.98, 0.84, 0.40, 0.05, 0.25, 0.85, 0.22, 0.45, 
0.17, 0.10, 0.89, 0.43, 0.84, 0.12, 0.62, 0.64, 0.51, 0.78, 0.39, 0.67, 0.64, 0.32, 0.87, 0.81, 0.06, 0.05, 0.18, 0.62, 
0.79, 0.44, 0.87, 0.69, 0.59, 0.49, 0.86, 0.71, 0.64, 0.66, 0.13, 0.87, 0.96, 0.57, 0.53, 0.20, 0.99, 0.15, 0.48, 0.37, 
0.67, 0.35, 0.41, 0.71, 0.77, 0.95, 0.07, 0.07, 0.03, 0.40, 0.66, 0.82, 0.28, 0.50, 0.18, 0.65, 0.52, 0.24, 0.37, 0.67, 
%0.28, 0.78, 0.57, 0.60, 0.47, 0.67, 0.14, 0.06, 0.55, 0.10, 0.10, 0.19, 0.22, 0.82, 0.58, 0.48, 0.68, 0.87, 0.84, 0.69, 
%0.09, 0.88, 0.69, 0.81, 0.22, 0.11, 0.14, 0.22, 0.04, 0.77, 0.92, 0.92, 0.61, 0.38, 0.14, 0.81, 0.93, 0.17, 0.42, 0.30, 
%0.22, 0.39, 0.76, 0.79, 0.48, 0.74, 0.81, 0.39, 0.68, 0.54, 0.29, 0.48, 0.51, 0.45, 0.35, 0.31, 0.23, 0.09, 0.81, 0.76, 
%0.19, 0.30, 0.46, 0.13, 0.71, 0.81, 0.41, 0.10, 0.05, 0.86, 0.89, 0.95, 0.60, 0.17, 0.76, 0.03, 0.23, 0.49, 0.12, 0.28,
%0.94, 0.44, 0.39, 0.23, 0.25, 0.03, 0.59, 0.66, 0.40, 0.44, 0.02, 0.58, 0.02, 0.46, 0.02, 0.40, 0.57, 0.59, 0.56, 0.97
}}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/AggregationCNNGS/PathNodePositions.tex <==
\def \posXarray {{0.000, 0.516, 0.129, 0.258, 0.387, 0.645, 0.774, 0.903, 0.032, 0.065, 
0.097, 0.161, 0.194, 0.226, 0.290, 0.323, 0.355, 0.419, 0.452, 0.484, 
0.548, 0.581, 0.613, 0.677, 0.710, 0.742, 0.806, 0.839, 0.871, 0.935, 
0.968, 1.000, }}

\def \posYarray {{0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 
0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 
0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 
0.500, 0.500, }}

\input{../ToolsCNNGS/palettes/w3schools.tex}

==> figures/AggregationCNNGS/_fuse_hidden0002970600000022 <==
This is pdfTeX, Version 3.14159265-2.6-1.40.16 (TeX Live 2015/Debian) (preloaded format=pdflatex 2018.2.13)  26 MAR 2018 17:38
entering extended mode
 restricted \write18 enabled.
 %&-line parsing enabled.
**SelectionCNNGSLayer3Pool.tex
(./SelectionCNNGSLayer3Pool.tex
LaTeX2e <2016/02/01>
Babel <3.9q> and hyphenation patterns for 81 language(s) loaded.
(/usr/share/texlive/texmf-dist/tex/latex/standalone/standalone.cls
Document Class: standalone 2015/07/15 v1.2 Class to compile TeX sub-files stand
alone
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifluatex.sty
Package: ifluatex 2010/03/01 v1.3 Provides the ifluatex switch (HO)
Package ifluatex Info: LuaTeX not detected.
)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifpdf.sty
Package: ifpdf 2011/01/30 v2.3 Provides the ifpdf switch (HO)
Package ifpdf Info: pdfTeX in PDF mode is detected.
)
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty
Package: ifxetex 2010/09/12 v0.6 Provides ifxetex conditional
)
(/usr/share/texlive/texmf-dist/tex/latex/xkeyval/xkeyval.sty
Package: xkeyval 2014/12/03 v2.7a package option processing (HA)

(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkvutils.tex
\XKV@toks=\toks14
\XKV@tempa@toks=\toks15

(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/keyval.tex))
\XKV@depth=\count79
File: xkeyval.tex 2014/12/03 v2.7a key=value parser (HA)
))
\sa@internal=\count80
\c@sapage=\count81

(/usr/share/texlive/texmf-dist/tex/latex/standalone/standalone.cfg
File: standalone.cfg 2015/07/15 v1.2 Default configuration file for 'standalone
' class
)
(/usr/share/texlive/texmf-dist/tex/latex/base/article.cls
Document Class: article 2014/09/29 v1.4h Standard LaTeX document class
(/usr/share/texlive/texmf-dist/tex/latex/base/size10.clo
File: size10.clo 2014/09/29 v1.4h Standard LaTeX file (size option)
)
\c@part=\count82
\c@section=\count83
\c@subsection=\count84
\c@subsubsection=\count85
\c@paragraph=\count86
\c@subparagraph=\count87
\c@figure=\count88
\c@table=\count89
\abovecaptionskip=\skip41
\belowcaptionskip=\skip42
\bibindent=\dimen102
)
(/usr/share/texlive/texmf-dist/tex/latex/varwidth/varwidth.sty
Package: varwidth 2009/03/30 ver 0.92;  Variable-width minipages
\@vwid@box=\box26
\sift@deathcycles=\count90
\@vwid@loff=\dimen103
\@vwid@roff=\dimen104
)
\sa@box=\box27
)
(/usr/share/texlive/texmf-dist/tex/latex/xcolor/xcolor.sty
Package: xcolor 2007/01/21 v2.11 LaTeX color extensions (UK)

(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/color.cfg
File: color.cfg 2007/01/18 v1.5 color configuration of teTeX/TeXLive
)
Package xcolor Info: Driver file: pdftex.def on input line 225.

(/usr/share/texlive/texmf-dist/tex/latex/pdftex-def/pdftex.def
File: pdftex.def 2011/05/27 v0.06d Graphics/color for pdfTeX

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/infwarerr.sty
Package: infwarerr 2010/04/08 v1.3 Providing info/warning/error messages (HO)
)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ltxcmds.sty
Package: ltxcmds 2011/11/09 v1.22 LaTeX kernel commands for general use (HO)
)
\Gread@gobject=\count91
)
Package xcolor Info: Model `cmy' substituted by `cmy0' on input line 1337.
Package xcolor Info: Model `hsb' substituted by `rgb' on input line 1341.
Package xcolor Info: Model `RGB' extended on input line 1353.
Package xcolor Info: Model `HTML' substituted by `rgb' on input line 1355.
Package xcolor Info: Model `Hsb' substituted by `hsb' on input line 1356.
Package xcolor Info: Model `tHsb' substituted by `hsb' on input line 1357.
Package xcolor Info: Model `HSB' substituted by `hsb' on input line 1358.
Package xcolor Info: Model `Gray' substituted by `gray' on input line 1359.
Package xcolor Info: Model `wave' substituted by `hsb' on input line 1360.
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.tex
\pgfutil@everybye=\toks16
\pgfutil@tempdima=\dimen105
\pgfutil@tempdimb=\dimen106

(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-lists.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
\pgfutil@abb=\box28
(/usr/share/texlive/texmf-dist/tex/latex/ms/everyshi.sty
Package: everyshi 2001/05/15 v3.00 EveryShipout Package (MS)
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
Package: pgfrcs 2015/08/07 v3.0.1a (rcs-revision 1.31)
))
Package: pgf 2015/08/07 v3.0.1a (rcs-revision 1.15)

(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
Package: graphicx 2014/10/28 v1.0g Enhanced LaTeX Graphics (DPC,SPQR)

(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
Package: graphics 2016/01/03 v1.0q Standard LaTeX Graphics (DPC,SPQR)

(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty
Package: trig 2016/01/03 v1.10 sin cos tan (DPC)
)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/graphics.cfg
File: graphics.cfg 2010/04/23 v1.9 graphics configuration of TeX Live
)
Package graphics Info: Driver file: pdftex.def on input line 95.
)
\Gin@req@height=\dimen107
\Gin@req@width=\dimen108
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
Package: pgfsys 2014/07/09 v3.0.1a (rcs-revision 1.48)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
\pgfkeys@pathtoks=\toks17
\pgfkeys@temptoks=\toks18

(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.code.t
ex
\pgfkeys@tmptoks=\toks19
))
\pgf@x=\dimen109
\pgf@y=\dimen110
\pgf@xa=\dimen111
\pgf@ya=\dimen112
\pgf@xb=\dimen113
\pgf@yb=\dimen114
\pgf@xc=\dimen115
\pgf@yc=\dimen116
\w@pgf@writea=\write3
\r@pgf@reada=\read1
\c@pgf@counta=\count92
\c@pgf@countb=\count93
\c@pgf@countc=\count94
\c@pgf@countd=\count95
\t@pgf@toka=\toks20
\t@pgf@tokb=\toks21
\t@pgf@tokc=\toks22
 (/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg
File: pgf.cfg 2008/05/14  (rcs-revision 1.7)
)
Driver file for pgf: pgfsys-pdftex.def

(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.def
File: pgfsys-pdftex.def 2014/10/11  (rcs-revision 1.35)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-pdf.de
f
File: pgfsys-common-pdf.def 2013/10/10  (rcs-revision 1.13)
)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.code.
tex
File: pgfsyssoftpath.code.tex 2013/09/09  (rcs-revision 1.9)
\pgfsyssoftpath@smallbuffer@items=\count96
\pgfsyssoftpath@bigbuffer@items=\count97
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.code.
tex
File: pgfsysprotocol.code.tex 2006/10/16  (rcs-revision 1.4)
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
Package: pgfcore 2010/04/11 v3.0.1a (rcs-revision 1.7)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex
\pgfmath@dimen=\dimen117
\pgfmath@count=\count98
\pgfmath@box=\box29
\pgfmath@toks=\toks23
\pgfmath@stack@operand=\toks24
\pgfmath@stack@operation=\toks25
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigonomet
ric.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.random.cod
e.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.comparison
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integerari
thmetics.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex
\c@pgfmathroundto@lastzeros=\count99
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.code.te
x
File: pgfcorepoints.code.tex 2013/10/07  (rcs-revision 1.27)
\pgf@picminx=\dimen118
\pgf@picmaxx=\dimen119
\pgf@picminy=\dimen120
\pgf@picmaxy=\dimen121
\pgf@pathminx=\dimen122
\pgf@pathmaxx=\dimen123
\pgf@pathminy=\dimen124
\pgf@pathmaxy=\dimen125
\pgf@xx=\dimen126
\pgf@xy=\dimen127
\pgf@yx=\dimen128
\pgf@yy=\dimen129
\pgf@zx=\dimen130
\pgf@zy=\dimen131
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconstruct.
code.tex
File: pgfcorepathconstruct.code.tex 2013/10/07  (rcs-revision 1.29)
\pgf@path@lastx=\dimen132
\pgf@path@lasty=\dimen133
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage.code
.tex
File: pgfcorepathusage.code.tex 2014/11/02  (rcs-revision 1.24)
\pgf@shorten@end@additional=\dimen134
\pgf@shorten@start@additional=\dimen135
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.code.te
x
File: pgfcorescopes.code.tex 2015/05/08  (rcs-revision 1.46)
\pgfpic=\box30
\pgf@hbox=\box31
\pgf@layerbox@main=\box32
\pgf@picture@serial@count=\count100
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicstate.c
ode.tex
File: pgfcoregraphicstate.code.tex 2014/11/02  (rcs-revision 1.12)
\pgflinewidth=\dimen136
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransformation
s.code.tex
File: pgfcoretransformations.code.tex 2015/08/07  (rcs-revision 1.20)
\pgf@pt@x=\dimen137
\pgf@pt@y=\dimen138
\pgf@pt@temp=\dimen139
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.code.tex
File: pgfcorequick.code.tex 2008/10/09  (rcs-revision 1.3)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.code.t
ex
File: pgfcoreobjects.code.tex 2006/10/11  (rcs-revision 1.2)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathprocessing
.code.tex
File: pgfcorepathprocessing.code.tex 2013/09/09  (rcs-revision 1.9)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.code.te
x
File: pgfcorearrows.code.tex 2015/05/14  (rcs-revision 1.43)
\pgfarrowsep=\dimen140
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.code.tex
File: pgfcoreshade.code.tex 2013/07/15  (rcs-revision 1.15)
\pgf@max=\dimen141
\pgf@sys@shading@range@num=\count101
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.code.tex
File: pgfcoreimage.code.tex 2013/07/15  (rcs-revision 1.18)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.code.
tex
File: pgfcoreexternal.code.tex 2014/07/09  (rcs-revision 1.21)
\pgfexternal@startupbox=\box33
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.code.te
x
File: pgfcorelayers.code.tex 2013/07/18  (rcs-revision 1.7)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransparency.c
ode.tex
File: pgfcoretransparency.code.tex 2013/09/30  (rcs-revision 1.5)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.code.
tex
File: pgfcorepatterns.code.tex 2013/11/07  (rcs-revision 1.5)
)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex
File: pgfmoduleshapes.code.tex 2014/03/21  (rcs-revision 1.35)
\pgfnodeparttextbox=\box34
) (/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.tex
File: pgfmoduleplot.code.tex 2015/08/03  (rcs-revision 1.13)
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-0-65
.sty
Package: pgfcomp-version-0-65 2007/07/03 v3.0.1a (rcs-revision 1.7)
\pgf@nodesepstart=\dimen142
\pgf@nodesepend=\dimen143
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-1-18
.sty
Package: pgfcomp-version-1-18 2007/07/23 v3.0.1a (rcs-revision 1.1)
)) (/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
Package: pgffor 2013/12/13 v3.0.1a (rcs-revision 1.25)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)
\pgffor@iter=\dimen144
\pgffor@skip=\dimen145
\pgffor@stack=\toks26
\pgffor@toks=\toks27
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.code.tex
Package: tikz 2015/08/07 v3.0.1a (rcs-revision 1.151)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothandlers
.code.tex
File: pgflibraryplothandlers.code.tex 2013/08/31 v3.0.1a (rcs-revision 1.20)
\pgf@plot@mark@count=\count102
\pgfplotmarksize=\dimen146
)
\tikz@lastx=\dimen147
\tikz@lasty=\dimen148
\tikz@lastxsaved=\dimen149
\tikz@lastysaved=\dimen150
\tikzleveldistance=\dimen151
\tikzsiblingdistance=\dimen152
\tikz@figbox=\box35
\tikz@figbox@bg=\box36
\tikz@tempbox=\box37
\tikz@tempbox@bg=\box38
\tikztreelevel=\count103
\tikznumberofchildren=\count104
\tikznumberofcurrentchild=\count105
\tikz@fig@count=\count106

(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.code.tex
File: pgfmodulematrix.code.tex 2013/09/17  (rcs-revision 1.8)
\pgfmatrixcurrentrow=\count107
\pgfmatrixcurrentcolumn=\count108
\pgf@matrix@numberofcolumns=\count109
)
\tikz@expandcount=\count110

(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibrarytopaths.code.tex
File: tikzlibrarytopaths.code.tex 2008/06/17 v3.0.1a (rcs-revision 1.2)
)))
(/usr/share/texlive/texmf-dist/tex/latex/subfigure/subfigure.sty
Package: subfigure 2002/03/15 v2.1.5 subfigure package
\subfigtopskip=\skip43
\subfigcapskip=\skip44
\subfigcaptopadj=\dimen153
\subfigbottomskip=\skip45
\subfigcapmargin=\dimen154
\subfiglabelskip=\skip46
\c@subfigure=\count111
\c@lofdepth=\count112
\c@subtable=\count113
\c@lotdepth=\count114

****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/share/texlive/texmf-dist/tex/latex/subfigure/subfigure.cfg)
\subfig@top=\skip47
\subfig@bottom=\skip48
)
(./SelectionCNNGSLayer3Pool.aux)
\openout1 = `SelectionCNNGSLayer3Pool.aux'.

LaTeX Font Info:    Checking defaults for OML/cmm/m/it on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for T1/cmr/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for OT1/cmr/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for OMS/cmsy/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for OMX/cmex/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for U/cmr/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.

(/usr/share/texlive/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
\scratchcounter=\count115
\scratchdimen=\dimen155
\scratchbox=\box39
\nofMPsegments=\count116
\nofMParguments=\count117
\everyMPshowfont=\toks28
\MPscratchCnt=\count118
\MPscratchDim=\dimen156
\MPnumerator=\count119
\makeMPintoPDFobject=\count120
\everyMPtoPDFconversion=\toks29
) ABD: EveryShipout initializing macros
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/pdftexcmds.sty
Package: pdftexcmds 2011/11/29 v0.20 Utility functions of pdfTeX for LuaTeX (HO
)
Package pdftexcmds Info: LuaTeX not detected.
Package pdftexcmds Info: \pdf@primitive is available.
Package pdftexcmds Info: \pdf@ifprimitive is available.
Package pdftexcmds Info: \pdfdraftmode found.
)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
Package: epstopdf-base 2010/02/09 v2.5 Base part for package epstopdf

(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/grfext.sty
Package: grfext 2010/08/19 v1.1 Manage graphics extensions (HO)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/kvdefinekeys.sty
Package: kvdefinekeys 2011/04/07 v1.3 Define keys (HO)
))
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/kvoptions.sty
Package: kvoptions 2011/06/30 v3.11 Key value format for package options (HO)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/kvsetkeys.sty
Package: kvsetkeys 2012/04/25 v1.16 Key value parser (HO)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/etexcmds.sty
Package: etexcmds 2011/02/16 v1.5 Avoid name clashes with e-TeX commands (HO)
Package etexcmds Info: Could not find \expanded.
(etexcmds)             That can mean that you are not using pdfTeX 1.50 or
(etexcmds)             that some package has redefined \expanded.
(etexcmds)             In the latter case, load this package earlier.
)))
Package grfext Info: Graphics extension search list:
(grfext)             [.png,.pdf,.jpg,.mps,.jpeg,.jbig2,.jb2,.PNG,.PDF,.JPG,.JPE
G,.JBIG2,.JB2,.eps]
(grfext)             \AppendGraphicsExtensions on input line 452.

(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg
File: epstopdf-sys.cfg 2010/07/13 v1.3 Configuration of (r)epstopdf for TeX Liv
e
))
(./SelectionCNNGSParam.tex (../ToolsCNNGS/DrawFeatures.tex)
(../ToolsCNNGS/ChooseNodeColor.tex) (../ToolsCNNGS/DrawGraphNodes.tex)
(../ToolsCNNGS/DrawGraphEdges.tex (../ToolsCNNGS/AuxMacrosDrawEdges.tex))
\pgf@layerbox@NodeLayer=\box40
\pgf@layerboxsaved@NodeLayer=\box41
\pgf@layerbox@EdgeLayer=\box42
\pgf@layerboxsaved@EdgeLayer=\box43
\pgf@layerbox@GNNLayerLayer=\box44
\pgf@layerboxsaved@GNNLayerLayer=\box45

(./NodePositions.tex))
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
LaTeX Font Info:    External font `cmex10' loaded for size
(Font)              <7> on input line 72.
LaTeX Font Info:    External font `cmex10' loaded for size
(Font)              <5> on input line 72.
 [1

] (./SelectionCNNGSLayer3Pool.aux) ) 
Here is how much of TeX's memory you used:
 12480 strings out of 493029
 251718 string characters out of 6136234
 370574 words of memory out of 5000000
 15781 multiletter control sequences out of 15000+600000
 3640 words of font info for 14 fonts, out of 8000000 for 9000
 1141 hyphenation exceptions out of 8191
 55i,10n,66p,427b,857s stack positions out of 5000i,500n,10000p,200000b,80000s

Output written on SelectionCNNGSLayer3Pool.pdf (1 page, 7393 bytes).
PDF statistics:
 11 PDF objects out of 1000 (max. 8388607)
 7 compressed objects within 1 object stream
 0 named destinations out of 1000 (max. 500000)
 13 words of extra memory for PDF output out of 10000 (max. 10000000)



==> figures/AggregationCNNGS/_fuse_hidden0002970700000021 <==
\relax 


==> figures/RegularCNN/DrawGraphNodes.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodes}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired
      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position 
   \clip (-0.1+\XposO,-0.2+\YposO) rectangle 
   		(\widthI+0.2-0.1+\XposO, 
   		\heightI+0.3-0.1+\YposO);
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity]    % Node opacity
             (\posX cm, \posY cm)            % Node position
             circle (\localNodeSize pt);     % Node size

\end{pgfonlayer}       
}
}


==> figures/RegularCNN/DrawGraphNodesR.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodesR}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired
      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position 
     \clip (-0.1+\XposO,-0.1+\YposO) rectangle 
   		(\widthI+0.2-0.1+\XposO, 
   		\heightI+0.2-0.1+\YposO);
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity,    % Node opacity
             rounded corners]
             (\posX cm - \localNodeSize pt, \posY cm - \localNodeSize pt)            % Node position
             rectangle (\posX cm + \localNodeSize pt, \posY cm + \localNodeSize pt);     % Node size

\end{pgfonlayer}       
}
}


==> figures/RegularCNN/RegularCNNParamLayer1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{4}
\def\Yscale{0.125}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphNodesR.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{RegularNodePositionsLayer1.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {16} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {40/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.01}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {8}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {8}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {0.57*\Radius}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {1.25*\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {4}                  % Number of nodes sample
\pgfmathsetmacro \twoNrPooledNodes       {4}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {1.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.3*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.2*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/RegularCNN/RegularCNNParamLayer2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{4}
\def\Yscale{1}

\def\XposO{0.267*\Xscale} % X position of first node (Origin)
\def\YposO{0.5*\Yscale} % Y position of first node (Origin)
\def\widthI{0.733*\Xscale-\XposO} % Width of image
\def\heightI{0.5*\Yscale-\YposO} % Height of image

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{DrawGraphNodes.tex}
\input{DrawGraphNodesR.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{RegularNodePositionsLayer2.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {8} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {20} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {8}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {8}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {2}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {2}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {1.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.2*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/RegularCNN/RegularCNNParamLayer3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{4}
\def\Yscale{0.125}

\def\XposO{0.455*\Xscale} % X position of first node (Origin)
\def\YposO{0.5*\Yscale} % Y position of first node (Origin)
\def\widthI{0.545*\Xscale-\XposO} % Width of image
\def\heightI{0.5*\Yscale-\YposO} % Height of image

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{DrawGraphNodes.tex}
\input{DrawGraphNodesR.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{RegularNodePositionsLayer3.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {2} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {50} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {2}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {2}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {2}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {2}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {4.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.25*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {0.35*\LargeConvSize} % Size of large1 convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/RegularCNN/RegularNodePositionsLayer1.tex <==
\def \posXarray {{
0.000,
0.133,
0.267, 
0.400, 
0.533, 
0.667,
0.800,  
0.933, 
0.067, 
0.200, 
0.333, 
0.467, 
0.600, 
0.733, 
0.867,   
1.000, }}

\def \posYarray {{0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 
0.500, 0.500, 0.500, 0.500, 0.500, 0.500, }}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/RegularCNN/RegularNodePositionsLayer2.tex <==
\def \posXarray {{
0.267,
0.533, 
0.333, 
0.400, 
0.467, 
0.600, 
0.667,
0.733, 
 }}

\def \posYarray {{ 0.500, 0.500, 
0.500, 0.500, 0.500, 0.500, 0.500, 0.500, }}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/RegularCNN/RegularNodePositionsLayer3.tex <==
\def \posXarray {{
0.455,
0.545,
}}

\def \posYarray {{0.5,
0.5,
}}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/RegularCNNGS/RegularCNNGSParam.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphNodesR.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{RegularNodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {96} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {40/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {12}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {12}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {1.5*\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {2}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {2}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {3*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {2.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {4*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {3*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/RegularCNNGS/RegularNodePositions.tex <==
\def \posXarray {{0.364, 0.636,
0.091, 0.091, 0.091, 0.364, 0.364, 0.636, 0.636, 0.909, 
0.909, 0.909, 0.000, 0.000, 0.000, 0.000, 0.000, 0.000, 0.000, 0.000, 
0.091, 0.091, 0.091, 0.091, 0.091, 0.182, 0.182, 0.182, 0.182, 0.182, 
0.182, 0.182, 0.182, 0.273, 0.273, 0.273, 0.273, 0.273, 0.273, 0.273, 
0.273, 0.364, 0.364, 0.364, 0.364, 0.364, 0.455, 0.455, 0.455, 0.455, 
0.455, 0.455, 0.455, 0.455, 0.545, 0.545, 0.545, 0.545, 0.545, 0.545, 
0.545, 0.545, 0.636, 0.636, 0.636, 0.636, 0.636, 0.727, 0.727, 0.727, 
0.727, 0.727, 0.727, 0.727, 0.727, 0.818, 0.818, 0.818, 0.818, 0.818, 
0.818, 0.818, 0.818, 0.909, 0.909, 0.909, 0.909, 0.909, 1.000, 1.000, 
1.000, 1.000, 1.000, 1.000, 1.000, 1.000, }}

\def \posYarray {{0.571, 0.571,
0.143, 0.571, 1.000, 0.143, 1.000, 0.143, 1.000, 0.143, 
0.571, 1.000, 0.000, 0.143, 0.286, 0.429, 0.571, 0.714, 0.857, 1.000, 
0.000, 0.286, 0.429, 0.714, 0.857, 0.000, 0.143, 0.286, 0.429, 0.571, 
0.714, 0.857, 1.000, 0.000, 0.143, 0.286, 0.429, 0.571, 0.714, 0.857, 
1.000, 0.000, 0.286, 0.429, 0.714, 0.857, 0.000, 0.143, 0.286, 0.429, 
0.571, 0.714, 0.857, 1.000, 0.000, 0.143, 0.286, 0.429, 0.571, 0.714, 
0.857, 1.000, 0.000, 0.286, 0.429, 0.714, 0.857, 0.000, 0.143, 0.286, 
0.429, 0.571, 0.714, 0.857, 1.000, 0.000, 0.143, 0.286, 0.429, 0.571, 
0.714, 0.857, 1.000, 0.000, 0.286, 0.429, 0.714, 0.857, 0.000, 0.143, 
0.286, 0.429, 0.571, 0.714, 0.857, 1.000, }}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/SelectionCNNGS/NodePositions.tex <==
\def \posXarray {{
0.47, 0.22, 0.78, 0.09, 0.81, 
0.63, 0.90, 0.99, 0.77, 0.70, 0.01, 0.61, 0.55, 0.04, 0.72, 0.98, 0.68, 0.57, 0.26, 0.23, 0.28, 0.06, 0.85, 0.89, 0.98, 
0.88, 0.26, 0.02, 0.14, 0.17, 0.20, 0.01, 0.68, 0.77, 0.05, 0.60, 0.60, 0.04, 0.50, 0.05, 0.49, 0.38, 0.85, 0.48, 0.49, 
0.28, 0.26, 0.80, 0.84, 0.71, 0.36, 0.22, 0.33, 0.10, 0.99, 0.04, 0.66, 0.20, 0.91, 0.21, 0.04, 0.26, 0.16, 0.25, 0.68, 
0.89, 0.92, 0.25, 0.45, 0.77, 0.31, 0.99, 0.09, 0.41, 0.45, 0.63, 0.19, 0.28, 0.58, 0.28, 0.72, 0.25, 0.80, 0.26, 0.61, 
0.19, 0.16, 0.09, 0.32, 0.08, 0.39, 0.04, 0.93, 0.83, 0.72, 0.81, 0.38, 0.94, 0.42, 0.66, 0.88, 0.30, 0.77, 0.58, 0.68, 
%0.64, 0.09, 0.35, 0.30, 0.75, 0.44, 0.40, 0.47, 0.77, 0.29, 0.41, 0.64, 0.27, 0.18, 0.77, 0.98, 0.97, 0.05, 0.45, 0.28, 
%0.65, 0.30, 0.17, 0.69, 0.60, 0.22, 0.68, 0.05, 0.61, 0.50, 0.50, 0.46, 0.76, 0.13, 0.73, 0.53, 0.31, 0.66, 0.49, 0.63, 
%0.35, 0.24, 0.81, 0.75, 0.37, 0.58, 0.57, 0.48, 0.73, 0.89, 0.16, 0.62, 0.44, 0.53, 0.82, 0.80, 0.02, 0.92, 0.16, 0.12, 
%0.19, 0.66, 0.75, 0.48, 0.17, 0.49, 0.50, 0.02, 0.40, 0.70, 0.39, 0.20, 0.32, 0.52, 0.31, 0.76, 0.29, 0.51, 0.66, 0.80, 
%0.16, 0.65, 0.13, 0.63, 0.35, 0.44, 0.06, 0.87, 0.23, 0.43, 0.13, 0.56, 0.36, 0.45, 0.25, 0.61, 0.26, 0.29, 0.99, 0.04
}}

\def \posYarray {{
0.52, 0.18, 0.22, 0.83, 0.78, 
0.03, 0.61, 0.08, 0.86, 0.33, 0.64, 0.99, 0.43, 0.50, 0.63, 0.63, 0.40, 0.51, 0.22, 0.06, 0.03, 0.19, 0.18, 0.23, 0.16, 
0.21, 0.19, 0.12, 0.35, 0.06, 0.28, 0.76, 0.66, 0.25, 0.62, 0.13, 0.72, 0.98, 0.84, 0.40, 0.05, 0.25, 0.85, 0.22, 0.45, 
0.17, 0.10, 0.89, 0.43, 0.84, 0.12, 0.62, 0.64, 0.51, 0.78, 0.39, 0.67, 0.64, 0.32, 0.87, 0.81, 0.06, 0.05, 0.18, 0.62, 
0.79, 0.44, 0.87, 0.69, 0.59, 0.49, 0.86, 0.71, 0.64, 0.66, 0.13, 0.87, 0.96, 0.57, 0.53, 0.20, 0.99, 0.15, 0.48, 0.37, 
0.67, 0.35, 0.41, 0.71, 0.77, 0.95, 0.07, 0.07, 0.03, 0.40, 0.66, 0.82, 0.28, 0.50, 0.18, 0.65, 0.52, 0.24, 0.37, 0.67, 
%0.28, 0.78, 0.57, 0.60, 0.47, 0.67, 0.14, 0.06, 0.55, 0.10, 0.10, 0.19, 0.22, 0.82, 0.58, 0.48, 0.68, 0.87, 0.84, 0.69, 
%0.09, 0.88, 0.69, 0.81, 0.22, 0.11, 0.14, 0.22, 0.04, 0.77, 0.92, 0.92, 0.61, 0.38, 0.14, 0.81, 0.93, 0.17, 0.42, 0.30, 
%0.22, 0.39, 0.76, 0.79, 0.48, 0.74, 0.81, 0.39, 0.68, 0.54, 0.29, 0.48, 0.51, 0.45, 0.35, 0.31, 0.23, 0.09, 0.81, 0.76, 
%0.19, 0.30, 0.46, 0.13, 0.71, 0.81, 0.41, 0.10, 0.05, 0.86, 0.89, 0.95, 0.60, 0.17, 0.76, 0.03, 0.23, 0.49, 0.12, 0.28,
%0.94, 0.44, 0.39, 0.23, 0.25, 0.03, 0.59, 0.66, 0.40, 0.44, 0.02, 0.58, 0.02, 0.46, 0.02, 0.40, 0.57, 0.59, 0.56, 0.97
}}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/SelectionCNNGS/SelectionCNNGSParam.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{NodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {100} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {80/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {30}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {5}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {5}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {3}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {1.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.2*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.7*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/graph_drawing_experiments/AuxMacrosDrawEdges.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro for computing distance between 2 points

\newcommand{\CalculateDistance}[2]
{
   \pgfmathsetmacro\Distance{ sqrt(     (#1)^2 +    (#2)^2 ) }; % Calculates 2-norm distance
%  \pgfmathsetmacro\Distance{      abs( (#1)   + abs(#2)   ) }; % Calculates 1-norm distance. May be faster
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro to get coordniates of a node
\makeatletter
\newcommand{\GetTikzXY}[3]{ 
    \tikz@scan@one@point\pgfutil@firstofone#1\relax
    \edef#2{\the\pgf@x}
    \edef#3{\the\pgf@y}
}
\makeatother



==> figures/graph_drawing_experiments/ChooseNodeColor.tex <==

% Macro for selecting node's color based on positions. The macro is not used in the final version. 
% Accepts as argument the (x,y) coordinate of the node.
% Returns the custom color currentcolor that can be used in color commands.

\newcommand{\ChooseNodeColor}[2]
{   
    % Store arguments of the function in readable variables
    \def\Xhere{#1}      
    \def\Yhere{#1}
    % Compute a color scale
    \pgfmathsetmacro{\thecurrentcolor}
                    { 0.8*exp( - 0.6*(abs(\Xhere-0.5) + abs(\Yhere-0.5)) }
    % Assign color scale according to colormap (Grayscale in current configuration}
    \definecolor{CurrentColor}{rgb}{\thecurrentcolor,\thecurrentcolor,\thecurrentcolor}
}



%\def\colors{{"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", 
%             "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%             "E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", 
%             "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%             "D5EAE7", "F3ELEB", "F6C4E1", "F79CD4"}} 
%
%\pgfmathsetmacro{\thecurrentcolor}{\colors[random(0,20)]}
%\definecolor{currentcolor}{HTML}{\thecurrentcolor}


==> figures/graph_drawing_experiments/DrawFeatures.tex <==

% Macro to draw a stack of features. 
% The first two parameters are the positions of the front feature. 
% The third and fourth two are the x and y offsets of subsequent features. 
% The fifth and sixth are the size of the features 
% The seventh parameter is the number of features
% The eight is the color of the feature plane

\newcommand{\DrawFeatures}[8]
{
   \pgfmathsetmacro\NumberFeatures {#7}    % The numb er of features is in the seventh parameter
   \foreach \i in {\NumberFeatures,...,1}  % Repeat number of features. Sweep backwards
   {
      \pgfmathsetmacro\FeaturePosX {(#3)*(\i-1)} % Offset x
      \pgfmathsetmacro\FeaturePosY {(#4)*(\i-1)} % Offset y     
      \path    (#1,           #2)          % Start position
            ++ (\FeaturePosX,\FeaturePosY) % Advance as per offset
       node[ draw, 
             rectangle, 
             black!70,
             anchor         = south west,
             fill           = #8, 
             minimum width  = #5,
             minimum height = #6    ]  {} ;
   }
}


==> figures/graph_drawing_experiments/DrawGraphEdges.tex <==
% Command to draw edges of a graph. The macro assumes that nodes have been 
% placed and that they have received tikZ labels of the form (a1), (a2), ..., (aN)
% This can be accomplished by loading the file DrawGraphNodes.tex:
%    \input{DrawGraphNodes.tex}
% and calling the macro DrawGraphNodes. The statement below draws nodes of a
% graph with 10 nodes and small circles for nodes:
%    \DrawGraphNodes {1}    % Start node
%                    {10}   % End node 
%                    {5}    % Node size
%                    {1}    % Opacity
%                    {0}    % X offset
%                    {0}    % Y offset

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    NrNodes: Number of nodes the graph has
%    Connectivity radius: How far aways to connect nodes  
%    Edge Color: A valid color to draw edges. E.g., gray!20.
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Load macros to get coordinate points and calculate distances
%
\input{AuxMacrosDrawEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphEdges}[7]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNrNodes     {#3}
\pgfmathsetmacro\localRadius      {#4}
\pgfmathsetmacro\localEdgeColor   {#5}
\pgfmathsetmacro\localOffsetX     {#6}
\pgfmathsetmacro\localOffsetY     {#7}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin loop for drawing graph edges. 
%% We sweep from \localStartNode to NrNodes drawing edges
%%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Draw node connections. We sweep through all nodes and check if they are close to \i
   % If the nodes are close, we draw an edge.
   \begin{pgfonlayer}{EdgeLayer} % Edges are drawn in the edge layer
      \GetTikzXY{(a\i)}{\NodePosX}{\NodePosY}; % Get coordinates of current node (node i)
      \pgfmathsetmacro\PreviousNode{\i -1} % A pgf technicality. Need to store index of previous node (\i-1)
      \foreach \j in {1,...,\localNrNodes} % Start loop sweeping through previous nodes
      {
         \GetTikzXY{(a\j)}{\OtherNodePosX}{\OtherNodePosY}; % Coordinates of the other node (node j)
         \CalculateDistance{\NodePosX-\OtherNodePosX}
                           {\NodePosY-\OtherNodePosY}; % Calculate distance between nodes i and j
         \ifdim \Distance cm < \localRadius cm % Check the nodes are close. 
            \draw[\localEdgeColor] (a\i) -- (a\j); %If they are close, draw and edge
         \fi 
      } % Close inner loop sweeping through previous nodes
   \end{pgfonlayer}      
} % Close main loop sweeping through nodes
}
 

==> figures/graph_drawing_experiments/DrawGraphNodes.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodes}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired

      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position   
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity]    % Node opacity
             (\posX cm, \posY cm)            % Node position
             circle (\localNodeSize pt);     % Node size
\end{pgfonlayer}       
}
}


==> figures/graph_drawing_experiments/NodePositions.tex <==
\def \posXarray {{
0.47, 0.22, 0.78, 0.09, 0.81, 
0.63, 0.90, 0.99, 0.77, 0.70, 0.01, 0.61, 0.55, 0.04, 0.72, 0.98, 0.68, 0.57, 0.26, 0.23, 0.28, 0.06, 0.85, 0.89, 0.98, 
0.88, 0.26, 0.02, 0.14, 0.17, 0.20, 0.01, 0.68, 0.77, 0.05, 0.60, 0.60, 0.04, 0.50, 0.05, 0.49, 0.38, 0.85, 0.48, 0.49, 
0.28, 0.26, 0.80, 0.84, 0.71, 0.36, 0.22, 0.33, 0.10, 0.99, 0.04, 0.66, 0.20, 0.91, 0.21, 0.04, 0.26, 0.16, 0.25, 0.68, 
0.89, 0.92, 0.25, 0.45, 0.77, 0.31, 0.99, 0.09, 0.41, 0.45, 0.63, 0.19, 0.28, 0.58, 0.28, 0.72, 0.25, 0.80, 0.26, 0.61, 
0.19, 0.16, 0.09, 0.32, 0.08, 0.39, 0.04, 0.93, 0.83, 0.72, 0.81, 0.38, 0.94, 0.42, 0.66, 0.88, 0.30, 0.77, 0.58, 0.68, 
%0.64, 0.09, 0.35, 0.30, 0.75, 0.44, 0.40, 0.47, 0.77, 0.29, 0.41, 0.64, 0.27, 0.18, 0.77, 0.98, 0.97, 0.05, 0.45, 0.28, 
%0.65, 0.30, 0.17, 0.69, 0.60, 0.22, 0.68, 0.05, 0.61, 0.50, 0.50, 0.46, 0.76, 0.13, 0.73, 0.53, 0.31, 0.66, 0.49, 0.63, 
%0.35, 0.24, 0.81, 0.75, 0.37, 0.58, 0.57, 0.48, 0.73, 0.89, 0.16, 0.62, 0.44, 0.53, 0.82, 0.80, 0.02, 0.92, 0.16, 0.12, 
%0.19, 0.66, 0.75, 0.48, 0.17, 0.49, 0.50, 0.02, 0.40, 0.70, 0.39, 0.20, 0.32, 0.52, 0.31, 0.76, 0.29, 0.51, 0.66, 0.80, 
%0.16, 0.65, 0.13, 0.63, 0.35, 0.44, 0.06, 0.87, 0.23, 0.43, 0.13, 0.56, 0.36, 0.45, 0.25, 0.61, 0.26, 0.29, 0.99, 0.04
}}

\def \posYarray {{
0.52, 0.18, 0.22, 0.83, 0.78, 
0.03, 0.61, 0.08, 0.86, 0.33, 0.64, 0.99, 0.43, 0.50, 0.63, 0.63, 0.40, 0.51, 0.22, 0.06, 0.03, 0.19, 0.18, 0.23, 0.16, 
0.21, 0.19, 0.12, 0.35, 0.06, 0.28, 0.76, 0.66, 0.25, 0.62, 0.13, 0.72, 0.98, 0.84, 0.40, 0.05, 0.25, 0.85, 0.22, 0.45, 
0.17, 0.10, 0.89, 0.43, 0.84, 0.12, 0.62, 0.64, 0.51, 0.78, 0.39, 0.67, 0.64, 0.32, 0.87, 0.81, 0.06, 0.05, 0.18, 0.62, 
0.79, 0.44, 0.87, 0.69, 0.59, 0.49, 0.86, 0.71, 0.64, 0.66, 0.13, 0.87, 0.96, 0.57, 0.53, 0.20, 0.99, 0.15, 0.48, 0.37, 
0.67, 0.35, 0.41, 0.71, 0.77, 0.95, 0.07, 0.07, 0.03, 0.40, 0.66, 0.82, 0.28, 0.50, 0.18, 0.65, 0.52, 0.24, 0.37, 0.67, 
%0.28, 0.78, 0.57, 0.60, 0.47, 0.67, 0.14, 0.06, 0.55, 0.10, 0.10, 0.19, 0.22, 0.82, 0.58, 0.48, 0.68, 0.87, 0.84, 0.69, 
%0.09, 0.88, 0.69, 0.81, 0.22, 0.11, 0.14, 0.22, 0.04, 0.77, 0.92, 0.92, 0.61, 0.38, 0.14, 0.81, 0.93, 0.17, 0.42, 0.30, 
%0.22, 0.39, 0.76, 0.79, 0.48, 0.74, 0.81, 0.39, 0.68, 0.54, 0.29, 0.48, 0.51, 0.45, 0.35, 0.31, 0.23, 0.09, 0.81, 0.76, 
%0.19, 0.30, 0.46, 0.13, 0.71, 0.81, 0.41, 0.10, 0.05, 0.86, 0.89, 0.95, 0.60, 0.17, 0.76, 0.03, 0.23, 0.49, 0.12, 0.28,
%0.94, 0.44, 0.39, 0.23, 0.25, 0.03, 0.59, 0.66, 0.40, 0.44, 0.02, 0.58, 0.02, 0.46, 0.02, 0.40, 0.57, 0.59, 0.56, 0.97
}}


\def \NodeColors{{
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
}} 


==> figures/graph_drawing_experiments/mainSelectionGNNParam.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{DrawFeatures.tex}
\input{ChooseNodeColor.tex}
\input{DrawGraphNodes.tex}
\input{DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{NodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {20} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {80/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {30}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {5}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {5}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {3}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {2.7*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.3*\LargeConvSize} % Size of large convolution circles (pooling)

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.7*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.3*\LargeConvSize} % Size of large convolution circles (pooling)


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/graph_drawing_experiments/old/DrawGraph.tex <==
% Command to draw a random graph. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The Edge color is hard coded to light gray
% The size and shape of the node is also hard coded. They are 5pt circles

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The parameters passed to the macro are, in order: 
%    Number of nodes, 
%    Number of nodes sampled, 
%    Connectivity Radius of the graph
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph
% Code assumes number of sampled nodes is at least 2 and that total number of nodes is at least 3

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Define colors to draw nodes and edges of the graph
\definecolor{EdgeColor}{rgb}{0.9, 0.9, 0.9}  % Light gray
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, 
                       draw, 
%                       clip = {(\OffsetXLocal,\OffsetYLocal) rectangle (0.2,0.2)},
                       minimum width = \NodeSizeLocal pt,
                       opacity = 0.2,
                       inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraph}[5]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\def\NrNodesLocal           {#1} 
\def\ConnectivityRadiusLocal{#2}
\def\OffsetXLocal           {#3}
\def\OffsetYLocal           {#4}
\def\NodeSizeLocal          {#5}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Draw circle to represent the first graph node. 
% The first node is drawn close to the south east corner 
\pgfmathsetmacro \randX{\Xscale*(1 - 0.1)} % The x-coordinate of node 1
\pgfmathsetmacro \randY{\Yscale*(0 + 0.1)} % The y-coordinate of node 1
\pgfmathsetmacro \posX{\randX + \OffsetXLocal} % Have to move coordinates to offset position of graph
\pgfmathsetmacro \posY{\randY + \OffsetYLocal}
% Draw the node. We use the node layer. This has to be created outside of the macro as it
% needs to be global. NodeLayer must be on top of EdgeLayer.
\begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
   \ChooseNodeColor{\randX}{\randY}   % Choose color for node 
   \node[ GraphNode,                  % Draw the node using GraphNode specifications
          CurrentColor,               % Color for node border
          fill=CurrentColor]          % Color for node interior
          (a1)                        % Node label for future reference
          at (\posX cm, \posY cm) {}; % Node position
\end{pgfonlayer}       

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes that are sampled
% Since node 1 has been drawn, we sweep from 2 to NrNodesSampled nodes.
% We draw random points in the graph box 
%
\foreach \i in {1,...,\NrNodesLocal} 
{
   % Chose node position at random
   \pgfmathsetmacro \randX{\Xscale*rnd} % The x-coordinate of node 1
   \pgfmathsetmacro \randY{\Yscale*rnd} % The y-coordinate of node 1
   \pgfmathsetmacro \posX{\randX + \OffsetXLocal } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \OffsetYLocal }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      \ChooseNodeColor{\randX}{\randY}   % Choose color for node 
      \node[ GraphNode,                  % Draw the node using GraphNode specifications
          CurrentColor,               % Color for node border
          fill=CurrentColor]          % Color for node interior
          (a\i)                        % Node label for future reference
          at (\posX cm, \posY cm) {}; % Node position   
\end{pgfonlayer}       
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin loop for drawing graph edges. 
%% We sweep from 1 to NrNodes drawing random edges
%%
\foreach \i in {2,...,\NrNodesLocal} 
{
   % Draw node connections. We sweep through all past nodes and check if they are close
   % If the nodes are close, we draw an edge.
   \begin{pgfonlayer}{EdgeLayer} % Edges are drawn in the edge layer
      \gettikzxy{(a\i)}{\NodePosX}{\NodePosY}; % Get coordinates of current node (node i)
      \pgfmathsetmacro\PreviousNode{\i -1} % A pgf technicality. Need to store index of previous node (\i-1)
      \foreach \j in {1,...,\PreviousNode} % Start loop sweeping through previous nodes
      {
         \gettikzxy{(a\j)}{\OtherNodePosX}{\OtherNodePosY}; % Coordinates of the other node (node j)
         \CalculateDistance{\NodePosX-\OtherNodePosX}
                           {\NodePosY-\OtherNodePosY}; % Calculate distance between nodes i and j
         \ifdim \Distance cm < \ConnectivityRadiusLocal cm % Check the nodes are close. 
            \draw[EdgeColor] (a\i) -- (a\j); %If they are close, draw and edge
         \fi 
      } % Close inner loop sweeping through previous nodes
   \end{pgfonlayer}      
} % Close main loop sweeping through nodes

} % Close Macro

==> figures/graph_drawing_experiments/old/DrawGraphArray.tex <==
% Command to draw a random graph. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The Edge color is hard coded to light gray
% The size and shape of the node is also hard coded. They are 5pt circles

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The parameters passed to the macro are, in order: 
%    Number of nodes, 
%    Connectivity Radius of the graph
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph
% Code assumes number of sampled nodes is at least 2 and that total number of nodes is at least 3

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Define colors to draw nodes and edges of the graph
\definecolor{EdgeColor}{rgb}{0.9, 0.9, 0.9}  % Light gray
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, 
                       draw, 
                       minimum width = \NodeSizeLocal pt,
                       opacity = 0.8,
                       inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphArray}[5]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\def\NrNodesLocal           {#1} 
\def\ConnectivityRadiusLocal{#2}
\def\OffsetXLocal           {#3}
\def\OffsetYLocal           {#4}
\def\NodeSizeLocal          {#5}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes that are sampled
% We sweep from 1 to NrNodesSampled nodes.
% We draw random points in the graph box 
%
\foreach \i in {1,...,\NrNodesLocal} 
{
   % Chose node position at random
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \OffsetXLocal } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \OffsetYLocal }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      \ChooseNodeColor{\randX}{\randY}   % Choose color for node 
      \node[ GraphNode,                  % Draw the node using GraphNode specifications
             CurrentColor,               % Color for node border
             fill=CurrentColor]          % Color for node interior
             (a\i)                        % Node label for future reference
             at (\posX cm, \posY cm) {}; % Node position   
\end{pgfonlayer}       
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin loop for drawing graph edges. 
%% We sweep from 1 to NrNodes drawing random edges
%%
\foreach \i in {2,...,\NrNodesLocal} 
{
   % Draw node connections. We sweep through all past nodes and check if they are close
   % If the nodes are close, we draw an edge.
   \begin{pgfonlayer}{EdgeLayer} % Edges are drawn in the edge layer
      \gettikzxy{(a\i)}{\NodePosX}{\NodePosY}; % Get coordinates of current node (node i)
      \pgfmathsetmacro\PreviousNode{\i -1} % A pgf technicality. Need to store index of previous node (\i-1)
      \foreach \j in {1,...,\PreviousNode} % Start loop sweeping through previous nodes
      {
         \gettikzxy{(a\j)}{\OtherNodePosX}{\OtherNodePosY}; % Coordinates of the other node (node j)
         \CalculateDistance{\NodePosX-\OtherNodePosX}
                           {\NodePosY-\OtherNodePosY}; % Calculate distance between nodes i and j
         \ifdim \Distance cm < \ConnectivityRadiusLocal cm % Check the nodes are close. 
            \draw[EdgeColor] (a\i) -- (a\j); %If they are close, draw and edge
         \fi 
      } % Close inner loop sweeping through previous nodes
   \end{pgfonlayer}      
} % Close main loop sweeping through nodes

} % Close Macrozimulitus

==> figures/tikz_styles.tex <==
\tikzstyle{phantom vertex} = [ ellipse, 
                               anchor = center, 
                               minimum height = 0.06*\unit, 
                               minimum width  = 0.06*\unit,
                               inner sep=0pt,
                               anchor=center]
\tikzstyle{red vertex}   = [black, fill = red!20,   phantom vertex, draw]
\tikzstyle{black vertex} = [black, fill = black!20, phantom vertex, draw]
\tikzstyle{blue vertex}  = [black, fill = blue!20,  phantom vertex, draw]
\tikzstyle{green vertex} = [black, fill = green!20,  phantom vertex, draw]
\tikzstyle{vertex}       = [draw, phantom vertex]

\tikzstyle{point} = [ellipse, inner sep=0pt, draw, fill=white, anchor = center,
                     minimum height = 0.05*\unit, minimum width  = 0.05*\unit]

==> figures/toolscnngs/AuxMacrosDrawEdges.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro for computing distance between 2 points

\newcommand{\CalculateDistance}[2]
{
   \pgfmathsetmacro\Distance{ sqrt(     (#1)^2 +    (#2)^2 ) }; % Calculates 2-norm distance
%  \pgfmathsetmacro\Distance{      abs( (#1)   + abs(#2)   ) }; % Calculates 1-norm distance. May be faster
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro to get coordniates of a node
\makeatletter
\newcommand{\GetTikzXY}[3]{ 
    \tikz@scan@one@point\pgfutil@firstofone#1\relax
    \edef#2{\the\pgf@x}
    \edef#3{\the\pgf@y}
}
\makeatother



==> figures/toolscnngs/ChooseNodeColor.tex <==

% Macro for selecting node's color based on positions. The macro is not used in the final version. 
% Accepts as argument the (x,y) coordinate of the node.
% Returns the custom color currentcolor that can be used in color commands.

\newcommand{\ChooseNodeColor}[2]
{   
    % Store arguments of the function in readable variables
    \def\Xhere{#1}      
    \def\Yhere{#1}
    % Compute a color scale
    \pgfmathsetmacro{\thecurrentcolor}
                    { 0.8*exp( - 0.6*(abs(\Xhere-0.5) + abs(\Yhere-0.5)) }
    % Assign color scale according to colormap (Grayscale in current configuration}
    \definecolor{CurrentColor}{rgb}{\thecurrentcolor,\thecurrentcolor,\thecurrentcolor}
}



%\def\colors{{"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", 
%             "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%             "E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", 
%             "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%             "D5EAE7", "F3ELEB", "F6C4E1", "F79CD4"}} 
%
%\pgfmathsetmacro{\thecurrentcolor}{\colors[random(0,20)]}
%\definecolor{currentcolor}{HTML}{\thecurrentcolor}


==> figures/toolscnngs/DrawFeatures.tex <==

% Macro to draw a stack of features. 
% The first two parameters are the positions of the front feature. 
% The third and fourth two are the x and y offsets of subsequent features. 
% The fifth and sixth are the size of the features 
% The seventh parameter is the number of features
% The eight is the color of the feature plane

\newcommand{\DrawFeatures}[8]
{
   \pgfmathsetmacro\NumberFeatures {#7}    % The numb er of features is in the seventh parameter
   \foreach \i in {\NumberFeatures,...,1}  % Repeat number of features. Sweep backwards
   {
      \pgfmathsetmacro\FeaturePosX {(#3)*(\i-1)} % Offset x
      \pgfmathsetmacro\FeaturePosY {(#4)*(\i-1)} % Offset y  
      \path (#1,           #2)          % Start position
            ++ (\FeaturePosX,\FeaturePosY) % Advance as per offset
       node[draw, 
             rectangle, 
             black!70,
             anchor         = south west,
             fill           = #8, 
             minimum width  = #5,
             minimum height = #6    ]  {} ;
   }
}


==> figures/toolscnngs/DrawGraphEdges.tex <==
% Command to draw edges of a graph. The macro assumes that nodes have been 
% placed and that they have received tikZ labels of the form (a1), (a2), ..., (aN)
% This can be accomplished by loading the file DrawGraphNodes.tex:
%    \input{DrawGraphNodes.tex}
% and calling the macro DrawGraphNodes. The statement below draws nodes of a
% graph with 10 nodes and small circles for nodes:
%    \DrawGraphNodes {1}    % Start node
%                    {10}   % End node 
%                    {5}    % Node size
%                    {1}    % Opacity
%                    {0}    % X offset
%                    {0}    % Y offset

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    NrNodes: Number of nodes the graph has
%    Connectivity radius: How far aways to connect nodes  
%    Edge Color: A valid color to draw edges. E.g., gray!20.
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Load macros to get coordinate points and calculate distances
%
\input{../ToolsCNNGS/AuxMacrosDrawEdges}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphEdges}[7]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNrNodes     {#3}
\pgfmathsetmacro\localRadius      {#4}
\pgfmathsetmacro\localEdgeColor   {#5}
\pgfmathsetmacro\localOffsetX     {#6}
\pgfmathsetmacro\localOffsetY     {#7}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin loop for drawing graph edges. 
%% We sweep from \localStartNode to NrNodes drawing edges
%%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Draw node connections. We sweep through all nodes and check if they are close to \i
   % If the nodes are close, we draw an edge.
   \begin{pgfonlayer}{EdgeLayer} % Edges are drawn in the edge layer
      \GetTikzXY{(a\i)}{\NodePosX}{\NodePosY}; % Get coordinates of current node (node i)
      \pgfmathsetmacro\PreviousNode{\i -1} % A pgf technicality. Need to store index of previous node (\i-1)
      \foreach \j in {1,...,\localNrNodes} % Start loop sweeping through previous nodes
      {
         \GetTikzXY{(a\j)}{\OtherNodePosX}{\OtherNodePosY}; % Coordinates of the other node (node j)
         \CalculateDistance{\NodePosX-\OtherNodePosX}
                           {\NodePosY-\OtherNodePosY}; % Calculate distance between nodes i and j
         \ifdim \Distance cm < \localRadius cm % Check the nodes are close. 
            \draw[\localEdgeColor] (a\i) -- (a\j); %If they are close, draw and edge
         \fi 
      } % Close inner loop sweeping through previous nodes
   \end{pgfonlayer}      
} % Close main loop sweeping through nodes
}
 


==> figures/toolscnngs/DrawGraphNodes.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodes}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired
      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position 
     \clip  (-0.1,-0.1) rectangle (\Xscale + 0.1, \Yscale + 0.1);
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity]    % Node opacity
             (\posX cm, \posY cm)            % Node position
             circle (\localNodeSize pt);     % Node size

\end{pgfonlayer}       
}
}


==> figures/toolscnngs/DrawGraphNodesR.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodesR}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired
      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position 
     \clip  (-0.1,-0.1) rectangle (1.6, 1.1);
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity,    % Node opacity
             rounded corners]
             (\posX cm - \localNodeSize pt, \posY cm - \localNodeSize pt)            % Node position
             rectangle (\posX cm + \localNodeSize pt, \posY cm + \localNodeSize pt);     % Node size

\end{pgfonlayer}       
}
}


==> figures/toolscnngs/palettes/alejandro.tex <==
\def \NodeColors{{
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
}} 


==> figures/toolscnngs/palettes/w3schools.tex <==
\def \NodeColors{{
"A9A904", "2EA904", "A90404", "A92E04", "A95704", "A98004", "80A904", "57A904",  "04A904", "04A92E",
"04A957", "04A980", "04A9A9", "0480A9", "045EA7", "0457A9", "042EA9", "0404A9", "2E04A9", "5704A9",
"8004A9", "A904A9", "A90480", "A90457", "A9042E", 
"A90404", "A92E04", "A95704", "A98004", "A9A904", "80A904", "57A904", "2EA904", "04A904", "04A92E",
"04A957", "04A980", "04A9A9", "0480A9", "045EA7", "0457A9", "042EA9", "0404A9", "2E04A9", "5704A9",
"8004A9", "A904A9", "A90480", "A90457", "A9042E",
"A90404", "A92E04", "A95704", "A98004", "A9A904", "80A904", "57A904", "2EA904", "04A904", "04A92E",
"04A957", "04A980", "04A9A9", "0480A9", "045EA7", "0457A9", "042EA9", "0404A9", "2E04A9", "5704A9",
"8004A9", "A904A9", "A90480", "A90457", "A9042E",
"A90404", "A92E04", "A95704", "A98004", "A9A904", "80A904", "57A904", "2EA904", "04A904", "04A92E",
"04A957", "04A980", "04A9A9", "0480A9", "045EA7", "0457A9", "042EA9", "0404A9", "2E04A9", "5704A9",
"8004A9", "A904A9", "A90480", "A90457", "A9042E",
}} 


==> plots_stability/eigenvalues_graphon.tex <==
%!TEX root = ../stability.tex

\pgfplotsset{xtick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}

\def \frequencyresponse 
     {   0.8}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 1*\unit,
             xmin = 0, xmax=8,
             xtick = {0, 0.3, 1.03, 1.57, 
              2.63, 3, 4.24, 5.51, 6.72, 7.6, 8},
             xticklabels = {\black{\footnotesize $0$},
			                \blue{\footnotesize $\ \ \ldots$},
             				\blue{\footnotesize $\ \lam_8$}, 
                            \blue{\footnotesize $\ \lam_7$},
                            \blue{\footnotesize $\ \lam_6$}, 
                            \blue{\footnotesize $\ \lam_5$}, 
                            \blue{\footnotesize $\ \lam_4$}, 
                            \blue{\footnotesize $\ \lam_3$},
                            \blue{\footnotesize $\ \lam_2$}, 
                            \blue{\footnotesize $\ \lam_1$},
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {-1},
             typeset ticklabels with strut,
             enlarge x limits=false]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57, 
              2.63, 3, 4.24, 5.51, 6.72, 7.6}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\frequencyresponse};

%\addplot[ domain=-0.5:7.5, 
%          samples = 80, 
%          color = black,
%          line width = 1.2]
%         {\frequencyresponse};


\end{axis}
\end{tikzpicture}


%{-0.22, 0.25, 0.61, 1.05, 1.37, 2.11, 
%  2.43, 3.07, 3.67, 4.13, 4.31, 5.05, 
%  5.20, 6.00, 6.42, 7.00}



==> prelim-graphon.tex <==
%!TEX root = graphons.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We introduce the paper's notation and review graph signal processing concepts (subsection \ref{sbs:gsp}) and basic properties of graphons and convergent graph sequences (subsection \ref{sbs:graphon}). These concepts will be fundamental in the introduction of the WSP framework in Section \ref{sec:gft}, as well as in the convergence analyses carried out in Section \ref{sec:filters}.

\subsection{Graph Signal Processing} \label{sbs:gsp}
 
Graphs are triplets $\bbG = (\ccalV, \ccalE, \ccalW)$ where $\ccalV$ is a set of $n$ nodes, $\ccalE \subseteq n \times n$ is a set of edges  and $\ccalW: \ccalE \to \reals$ is a weight function assigning weights $\ccalW(i,j) = w_{ij}$ to edges $(i,j)$ in $\ccalE$. The graph $\bbG$ can also be represented by the graph shift operator (GSO) $\bbS \in \reals^{N \times N}$; the GSO is a matrix that captures the sparsity pattern of $\bbG$ by setting $[\bbS]_{ij} = s_{ij} \neq 0$ if and only if $i=j$ or $(j,i) \in \ccalE$. Examples of shift operators include: the adjacency matrix $\bbA$, where $[\bbA]_{ij} = w_{ji}$; the Laplacian matrix $\bbL = \bbD - \bbA$, where $\bbD = \bbA\mathbf{1}$; and their normalized counterparts. Throughout this paper, we will consider undirected graphs with $\bbS := \bbA$. The GSO will therefore always be symmetric, and, where convenient, will replace $\ccalW$ in the triplet notation $\bbG = (\ccalV, \ccalE, \bbS)$. 

We represent information on graphs as graph signals. Graph signals are maps from the vertex set $\ccalV$ onto the real numbers, which we write as pairs $(\bbG, \bbx)$ and where $[\bbx]_i$ is the value of the signal at node $i$. A number of graph operations can be defined on the signal $(\bbG, \bbx)$; the most basic one is the one induced by the GSO. This operation can be seen as a 1-step shift on the graph, which diffuses the information contained in each node to its 1-hop neighbors. Take the $i$th component of $\bbS\bbx$, for instance. In $[\bbS \bbx]_i = \sum_{j=1}^n s_{ij} x_j$, $s_{ij}$ is nonzero only if $i=j$ or $(i,j) \in \ccalE$. 

For $k>1$, the operators induced by $\bbS^k$ are defined analogously and have the effect of diffusing information up to $k$ hops away.
These operators can be further generalized to linear shift-invariant graph filters (LSI-GFs), which are order-$K$ polynomials of $\bbS$. We define a linear shift-invariant filter $\bbH(\bbS)$ as \cite{segarra17-linear}
\begin{equation} \label{eqn:lsi-gf}
\bbH(\bbS) \bbx = \sum_{k=0}^K h_k \bbS^k \bbx
\end{equation}
where the weights $h_0, \ldots, h_k$ are the graph filter's taps. This filter is shift-invariant because, if $\bby = \bbH(\bbS)\bbx$ and we shift the input to $\bbx' = \bbS\bbx$, the output $\bby' = \bbH(\bbS)\bbx'$ is simply the shifted version of $\bby$, $\bby' = \bbS\bby$.

Since $\bbS$ is symmetric, it is diagonalizable as $\bbS = \bbV \bbLam \bbV^{\Hr}$, where $\bbLam$ is the diagonal matrix of eigenvalues and the columns of $\bbV$ are the graph's eigenvectors. We define the Graph Fourier Transform (GFT) of the graph signal $(\bbG,\bbx)$ as 
\begin{equation} \label{eqn:gft}
\mbox{GFT} \{(\bbG, \bbx)\} := \hbx = \bbV^\Hr \bbx\ .
\end{equation}
This operation has the effect of decomposing $(\bbG, \bbx)$ in the eigenbasis of the graph, which makes sense if we interpret the eigenvalues as frequencies. The inverse Fourier Transform (iGFT) is defined as
\begin{equation}
\mbox{iGFT} \{\hbx\} := \bbV \hbx = \bbx\ .
\end{equation}
Since $\bbV^\Hr\bbV=\bbI$, the iGFT is a proper inverse and can recover $\bbx$ from $\hbx$ without loss of information.

Like graph signals, the linear graph filters from equation \eqref{eqn:lsi-gf} admit a spectral representation $\hbH(\bbLam)$,
\begin{equation} \label{eqn:lsi_graph_filter_resp}
\hbH(\bbLam)= \sum_{k=0}^K h_k \bbLam^k
\end{equation}
which is polynomial on the eigenvalues of the GSO. This is fortuitous, as polynomials can be used to approximate differentiable functions through their Taylor series expansion. Indeed, a filter with frequency response
\begin{equation} \label{eqn:any_graph_filter_resp}
\hbH(\lambda)= h(\lambda)
\end{equation}
can be approximated arbitrarily well by an LSI-GF at any $\lambda$ where $h$ is infinitely differentiable. Filters like the one in equation \eqref{eqn:any_graph_filter_resp} are sometimes referred to as \textit{spectral graph filters} \cite{elvin19-spectral} because of their explicit dependence on the eigenvalues (or spectrum) of the graph.

%This also means that they are linear in the eigenvalue powers $\Lambda^k$, which makes them unable discriminate between different eigenvalues --- $h_k$ is the same for $\lambda_i^k$ for all $i$. But this need not be the case; in particular, linear graph filters can be seen as part of a broader class of possibly nonlinear graph filters with the additional flexibility of being able to discriminate between different eigenvalues. These filters are called spectral graph filters (SGFs) and written as
%\begin{equation} \label{eqn:si-gf}
%\bbH(\bbS) \bbx = \sum_{k=0}^K \bbV h_k(\Lambda) \bbV^H \bbx
%\end{equation}
%where the $h_k$ are now ``filter tap functions'' satisfying $h_k(\Lambda ) = \diag ([h_k(\lambda_1), \ldots, h_k(\lambda_N)])$. From \eqref{eqn:si-gf}, the frequency response of the spectral graph filter $\bbH(\bbS)$ is easy to derive,
%\begin{equation} \label{eqn:si_graph_filter_resp}
%\hbH(\Lambda)= \sum_{k=0}^K h_k(\Lambda)
%\end{equation}
%and we conclude that, like \eqref{eqn:lsi_graph_filter_resp}, this expression still depends on the graph's eigenvalues, however this time modified by the functions $h_k$. Equations \eqref{eqn:lsi_graph_filter_resp} and \eqref{eqn:si_graph_filter_resp} are interesting because they show that the spectral behavior of both linear and spectral graph filters is solely determined by the graph's eigenvalues and by the filter's taps or tap functions, with no dependence on the graph's eigenvectors whatsoever. This property will be crucial in characterizing the frequency response of filters applied to convergent graph sequences in Section \ref{sec:filters}. 

\subsection{Graphons and Convergent Graph Sequences} \label{sbs:graphon}

\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.3\textwidth}
		\centering
		\includegraphics[height=3.5cm]{figures/sbm_graphon.pdf}
		\centering
		\includegraphics[height=3.2cm]{figures/sbm_graph.pdf}
		\caption{SBM with balanced communities} 
		\label{sbm1}
	\end{subfigure}
	\hspace{0.2cm}
	\begin{subfigure}{0.3\textwidth}
		\centering
		\includegraphics[height=3.5cm]{figures/sbm_graphon2.pdf}
		\centering
		\includegraphics[height=3.2cm]{figures/sbm_graph2.pdf} 
		\caption{SBM with imbalanced communities} 
		\label{sbm2}
	\end{subfigure}\hspace{0.2cm}
	\begin{subfigure}{0.3\textwidth}
		\centering
		\includegraphics[height=3.5cm]{figures/exp_graphon.pdf}
		\centering
		\includegraphics[height=3.2cm]{figures/exp_graph.pdf} 
		\caption{Exponential} 
		\label{exp}
	\end{subfigure}
	\caption{Graphons and $12$-node $\bbW$-random graphs sampled from them. Figures \subref{sbm1} and \subref{sbm2} show SBM graphons and graphs with 2 communities and $p_{c_i c_i} = 0.8, p_{c_i c_j} = 0.2$. Figure \subref{exp} shows an exponential graphon with expression $\bbW(x,y) = \exp (-2.3(x-y)^2)$ and the corresponding graph.}
	\label{fig:graphon_examples}
\end{figure*}	

A graphon is a bounded symmetric measurable function 
%
\begin{align}\label{eqn_graphon}
   \bbW: [0,1]^2 \to [0,1]. 
\end{align}
%
Equivalently, a graphon is a \textit{kernel} with range restricted to the unit interval and in either case it represents discrete graphs as infinite-dimensional analytic objects \cite{wolfe2013nonparametric}. In other words, a graphon is the representation of a graph with an uncountable number of nodes. By their very construction, graphons can be interpreted as probability distributions on the unit square. As such, we can sample $n$-node graphs $\bbG_n$ where every node $i \in [n]$ is associated with a sample point $u_i \in [0,1]$ and where the edges are defined either by assigning edge weight $\bbW(u_i,u_j)$ to edge $(i,j)$ or by connecting $i$ and $j$ with probability 
%
\begin{align}\label{eqn_sampled_graph}
   p_{ij} = \bbW(u_i,u_j).
\end{align}
%
In the latter case, the $\bbG_n$ are unweighted; if, additionally, the $u_i$ are sampled independently and uniformly at random, these graphs are called \textit{$\bbW$-random graphs}. Three examples of graphons and $W$-random graphs sampled from them are shown in Figure \ref{fig:graphon_examples}. The ones on the left (\ref{sbm1} and \ref{sbm2}) are SBM graphons with 2 communities, intra-community probability $0.8$ and inter-community probability $0.2$. The difference between them is that in \ref{sbm2} the communities are imbalanced. On the right (\ref{exp}), the graphon is exponential with expression $\bbW(u,v) = \exp (-2.3(u-v)^2)$.

A second and perhaps more interesting interpretation of graphons is as the limit objects of convergent graph sequences. A sequence of graphs $\{\bbG_n\}$ is said to converge if and only if the density of homomorphisms between any undirected and unweighted graph (or \textit{simple graph} for short) $\bbF = (\ccalV', \ccalE')$ and the $\bbG_n$ converges \cite{lovasz2006limits}. Homomorphisms between $\bbF$ and an arbitrary graph $\bbG = (\ccalV, \ccalE, \bbS)$ are adjacency preserving maps from $\ccalV$ to $\ccalV'$, that is, a map $\beta: \ccalV' \to \ccalV$ is an homomorphism if, for every $(i,j) \in \ccalE'$, $(\beta(i),\beta(j)) \in \ccalE$. The number of homomorphisms between $\bbF$ and $\bbG$ is denoted by $\mbox{hom}(\bbF, \bbG)$. There are a total of $|\ccalV|^{|\ccalV'|}$ possible maps between the vertices of $\bbF$ and $\bbG$, but since only a fraction of them are homomorphisms, we define the density of homomorphisms from $\bbF$ to $\bbG$ as \cite{lovasz2012large}
\begin{equation}
t(\bbF,\bbG) = \dfrac{\mbox{hom}(\bbF,\bbG)}{|\ccalV|^{|\ccalV'|}} := \dfrac{\sum_\beta \prod_{(i,j) \in \ccalE'} [\bbS]_{\beta(i) \beta(j)}}{|\ccalV|^{|\ccalV'|}}\ .
\end{equation}
This is easiest to understand in the case where $\bbG$ is unweighted, where $t(\bbF,\bbG)$ is simply the total number of ways in which $\bbF$ can be mapped into $\bbG$.

%\myparagraph{$\diamond$ Graph cut distances}

%\noindent \textit{Cut distance between two graphs on the same set of nodes.} Consider two graphs $\bbG = (\ccalV, \ccalE, \bbA)$ and $\bbG' = (\ccalV, \ccalE', \bbA')$ on the same set of $N$ nodes, where $\ccalE,\ccalE' \subseteq \ccalV \times \ccalV$ are the sets of edges and $\bbA,\bbA' \in \reals^{N \times N}$ are the adjacency matrices of $\bbG$ and $\bbG'$. Let $\ccalV_1$ and $\ccalV_2$ be sets such that $\ccalV_1,\ccalV_2 \subseteq \ccalV$, and denote by $E(\ccalV_1,\ccalV_2) = |\ccalE(\ccalV_1,\ccalV_2)|$ the number of edges with one endnode in $\ccalV_1$ and one in $\ccalV_2$. The cut distance between $\bbG$ and $\bbG'$ is defined as
%	\begin{equation}
%		d_{\square}(\bbG,\bbG') = \max_{\ccalV_1,\ccalV_2 \subseteq \ccalV} \dfrac{|E(\ccalV_1,\ccalV_2)-E'(\ccalV_1,\ccalV_2)|}{N^2}
%\end{equation}
%or, alternatively,
%	\begin{equation}
%		d_{\square}(\bbG,\bbG') = \|\bbA-\bbA'\|_\square 
%	\end{equation}
%where $\|\cdot\|_\square$ is the matrix cut norm \cite{alon2004approximating}.

%\noindent \textit{Cut distance between arbitrary graphs with $|\ccalV| = |\ccalV'| = N$.} Consider two arbitrary graphs of same size, $\bbG = (\ccalV,\ccalE,\bbA)$ and $\bbG' = (\ccalV', \ccalE', \bbA')$, where $|\ccalV| = |\ccalV'| = N$. The cut distance between $\bbG$ and $\bbG'$ is \cite{lovasz2012large}
%\begin{equation}
%\hat{\delta}_\square(\bbG,\bbG') = \min_{\hat{\bbG}, \hat{\bbG'}} d_\square(\hat{\bbG}, \hat{\bbG'})
%\end{equation}
%where $\hat{\bbG}, \hat{\bbG'}$ range over all permutations of $\bbG$ and $\bbG'$ respectively.

%\noindent \textit{Cut distance between two arbitrary graphs.} Consider two arbitrary graphs $\bbG = (\ccalV, \ccalE, \bbA)$ and $\bbG' = (\ccalV', \ccalE', \bbA')$ with $|\ccalV| = N$ and $|\ccalV'| = N'$. From $\bbG$ and $\bbG'$ and for $m \in \mbN^+$, we define the constructions $\bbG(m)$ and $\bbG'(m)$, where each node in $\bbG$ or $\bbG'$ is replaced by $m$ nodes, and two nodes in $\bbG(m)$ or $\bbG'(m)$ are connected by an edge only if there is an edge between their predecessors in $\bbG$ and $\bbG'$. The cut distance between $\bbG$ and $\bbG'$ is then \cite{lovasz2012large}
%begin{equation}
%\delta_\square(\bbG,\bbG') = \lim_{k \to \infty} \hat{\delta}_\square\left(\bbG(kN'),\bbG'(kN)\right)\ .
%\end{equation}

%\myparagraph{$\diamond$ Convergent graph sequences and graphons} 
The concept of homomorphism densities can also be generalized to graphons. We define the density of homomorphisms between the graph $\bbF$ and the graphon $\bbW$ as \cite{lovasz2012large}
\begin{equation}
t(\bbF,\bbW) = \int_{[0,1]^{\ccalV'}} \prod_{(i,j) \in \ccalE'} \bbW(u_i,u_j) \prod_{i \in \ccalV'} du_i\ .
\end{equation}
%\noindent \textit{Definition of convergence.} 
In the context of graph sequences, we then say that a sequence of undirected graphs $\{\bbG_n\}$ converges if and only if 
\begin{equation}
\lim_{n \to \infty} t(\bbF,\bbG_n) = t(\bbF, \bbW)
\end{equation}
in which case $\bbW$ is said to be the \textit{limit graphon} of the sequence. This form of convergence is called ``convergence in the homomorphism density sense''.

\begin{remark}[Convergent sequences of $\bbW$-random graphs] \label{rmk:w-random}
An example of convergent graph sequence that is easy to visualize is that of a sequence of $\bbW$-random graphs. The sequence of graphs $\{\bbG_n\}$ generated by sampling $\{u_i\}_{i=1}^n$ uniformly at random as $n \to \infty$ can be show to converge in the homomorphism density sense with probability 1. 
\end{remark}

\begin{remark}[Graphons induced by a graph] \label{rmk:graphon-induced}
Just like $\bbW$-random graphs can be sampled from a graphon $\bbW$, every undirected graph $\bbG_n = ([n], \ccalE_n, \bbS_n)$, where $\bbS_n$ is normalized by $n$, admits graphon representations $\bbW_\bbG$ obtained by constructing partitions $I_1 \cup \ldots \cup I_n$ of $[0,1]$ and setting 
\begin{equation}
\bbW_\bbG(u,v) = [\bbS]_{jk} \times \mbI(u \in I_j)\mbI(v \in I_k)\ .
\end{equation}
We refer to $\bbW_\bbG$ as 
the \textit{graphon induced by} $\bbG$.
%and will be of particular importance in the analysis of convergent graph sequences developed in upcoming section.
\end{remark}


